Is Network the Bottleneck of Distributed Training?

Recently there has been a surge of research on improving the communication efficiency of distributed training. However, little work has been done to systematically understand whether the network is the bottleneck and to what extent. In this paper, we take a first-principles approach to measure and analyze the network performance of distributed training. As expected, our measurement confirms that communication is the component that blocks distributed training from linear scale-out. However, contrary to the common belief, we find that the network is running at low utilization and that if the network can be fully utilized, distributed training can achieve a scaling factor of close to one. Moreover, while many recent proposals on gradient compression advocate over 100x compression ratio, we show that under full network utilization, there is no need for gradient compression in 100 Gbps network. On the other hand, a lower speed network like 10 Gbps requires only 2x--5x gradients compression ratio to achieve almost linear scale-out. Compared to application-level techniques like gradient compression, network-level optimizations do not require changes to applications and do not hurt the performance of trained models. As such, we advocate that the real challenge of distributed training is for the network community to develop high-performance network transport to fully utilize the network capacity and achieve linear scale-out.

==> Makefile <==
NAME=paper

TARGET=$(NAME)

all: $(TARGET).pdf

quick: Makefile *.tex sections/*.tex *.bib figures/*
	pdflatex  $(TARGET).tex
	rm -f *.aux *.log *.out *.bbl *.blg *~ *.bak $(FIGS) $(TARGET).ps $(TARGET).synctex.gz
	if which xdg-open 1>/dev/null 2>&1; then \
		xdg-open $(TARGET).pdf; \
	else \
		open -a Preview $(TARGET).pdf & \
	fi

$(TARGET).pdf: Makefile *.tex sections/*.tex *.bib figures/*
	pdflatex  $(TARGET).tex
	-bibtex --min-crossrefs=100    $(TARGET)
	pdflatex  $(TARGET).tex
	pdflatex  $(TARGET).tex
	rm -f *.aux *.log *.out *.bbl *.blg *~ *.bak $(FIGS) *.ps *.synctex.gz
	if which xdg-open 1>/dev/null 2>&1; then \
		xdg-open $(TARGET).pdf; \
	else \
		open -a Preview $(TARGET).pdf & \
	fi

clean:
	rm -f *.aux *.log *.out *.bbl *.blg *~ *.bak $(FIGS) *.ps *.pdf *.synctex.gz


==> sections/background.tex <==
\section{Background}

% In this section, we briefly review the distributed training process, parallelism strategies, communication framework, and distributed optimization algorithms.

% Intro to distributed training.
\subsection{Data Parallel Distributed Training}

During model training, the training progresses with a mini-batch of data samples in an iterative way. Each iteration consists of three steps: (1) forward propagation to compute the loss with model parameters and the data batch, (2) backward propagation to compute the gradient with regard to the loss, and (3) updates on the parameters based on the gradient and the optimization algorithm. Stochastic gradient descent (SGD) is one of the commonly used optimization algorithms, which updates the model parameters using the gradient estimated from the stochastic mini-batch to optimize the loss function in a iterative way. For distributed training, multiple workers participate to jointly complete the above three steps for each mini-batch. 

Algorithm \ref{algo:data_para} describes data parallel distributed training with synchronized (SGD), which is the most common framework for distributed training. In data parallel distributed training, the model parameter is replicated on all workers, and the data mini-batch is partitioned across the workers. In every iteration, each worker independently performs forward computation based on its data partition, followed by backward propagation to compute the gradient. To perform parameter update, gradient is synchronized and allreduced across all workers. Finally, each worker updates its copy of parameter based on the gradient with SGD. 

\begin{algorithm}[t!]
   \caption{Data parallel distributed training}
   \label{algo:data_para}
\begin{algorithmic}
   \STATE {\bfseries Notation:}  Dataset $X$, number of workers $N$, number of iterations $T$, model parameter $W$
   \FOR{iteration $t = 1$ {\bfseries to} $T$}
     \STATE Randomly sample mini-batch $x$\textasciitilde $X$, partition $N$-way
     \FOR{worker $i = 1$ {\bfseries to} $N$ \COMMENT{run in parallel}}
       \STATE Compute loss $l_i$ based on partition $x_i$ and $W_t$
       \STATE Compute gradient $g_{i}$ with regard to $l_i$
       \STATE Allreduce gradient by $g \gets \sum_{i=1}^N g_i$
       \STATE Update parameters by $W_{t+1} \gets sgd(W_{t}, g)$
     \ENDFOR
   \ENDFOR
\end{algorithmic}
\end{algorithm}

% All local gradients are averaged over workers through synchronous communication to obtain the global gradient for this mini-batch. Then this global gradient is used to update model parameters by the SGD update rule. Algorithm~\ref{algo:data_para} illustrates how a single batch is computed.
% Describe data parallelism vs. model parallelism vs. mixed data and model parallelism,


\subsection{Other Parallelism Strategies}
% Different parallelism strategies define how the work is divided among workers, while different distributed optimization algorithms imply different synchronization requirement between iterations. 

\parabf{Model Parallelism}

\parabf{Mixed Data and Model Parallelism}

\parabf{Pipeline Parallelism}

\subsection{Communication Framework}

\parabf{All-reduce} % MPI allreduce

\parabf{Parameter Server}

\subsection{Distributed Optimization Algorithms}

% Mini-batch stochastic gradient descent (SGD) with mo-mentum (e.g. heavy-ball momentum, Nesterov momentum,Adam [33,20]) is a widely used optimization method totrain deep learning models in computer vision.  Previouswork focuses on asynchronous SGD (asyncSGD) for environ-ments where machines are loosely coupled [5]. AsyncSGD,however, converges radically differently from synchronousmini-batch SGD [49,36,52].  It is also difficult for async-SGD to match the model accuracy trained with synchronizedmini-batch SGD with similar computation budget [5, 2]

\parabf{sync SGD}

\parabf{async SGD}

% \paragraph{Scheduler}
% The scheduler maintains the training state and coordinates the resources. It tracks the current and future number of workers and servers by monitoring existing workers and servers, as well as availability notices from the cluster resource provider. Furthermore, the scheduler keeps track of workloads (typically the range of data from which mini-batches are drawn) assigned to workers.
% \paragraph{Worker}
% Each worker computes the gradients per mini-batch and sends them to parameter servers. It then pulls updated parameters from parameter servers for the next mini-batch computation.
% \paragraph{Parameter Server}
% The parameter server for the training task maintains the copy of model parameters, updates the parameters based on the aggregated %performs the optimization based on  
% gradients from workers, and send the updated parameters back to workers. The parameters can be %from elasticity by
% partitioned among multiple machines with a distributed hash table\cite{byers2003simple}.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:

